Impact of Limpware on HDFS: A Probabilistic Estimation

With the advent of cloud computing, thousands of machines are connected and managed collectively. This era is confronted with a new challenge: performance variability, primarily caused by large-scale management issues such as hardware failures, software bugs, and configuration mistakes. In our previous work we highlighted one overlooked cause: limpware - hardware whose performance degrades significantly compared to its specification. We showed that limpware can cause severe impact in current scale-out systems. In this report, we quantify how often these scenarios happen in Hadoop Distributed File System.

==> Makefile <==
MAIN      = main
SRCS      = *.tex 
PS        = $(MAIN).ps
PDF       = $(MAIN).pdf
DVI       = $(MAIN).dvi
TARG      = $(MAIN).done



#all: texwithredo cleanabit
all: texnoredo cleanabit


p: all ps pdf skim cleanabit

skim:
	${HOME}/bin/skim main.pdf


f:
	latex freq.tex
	bibtex -min-crossrefs=100 freq
	${HOME}/bin/redo-bib.csh freq
	latex freq.tex
	latex freq.tex
	dvips -o freq.ps freq.dvi
	ps2pdf14 freq.ps 
	rm -vf *.ps  *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png
	${HOME}/bin/skim freq.pdf

sf: 
	${HOME}/bin/skim freq.pdf	


texwithredo:
	latex main.tex
	bibtex -min-crossrefs=100 main
	${HOME}/bin/redo-bib.csh main
	latex main.tex
	latex main.tex

texnoredo:
	latex main.tex
	bibtex -min-crossrefs=100 main
	latex main.tex
	latex main.tex



$(MAIN).bbl: $(MAIN).aux
	bibtex -min-crossrefs=100 $(MAIN)
	./redo-bib.csh $(MAIN)


$(MAIN).aux: $(MAIN).tex
	latex $(MAIN)

ps:
	dvips -o $(PS) $(MAIN)

pdf:
	ps2pdf14 $(PS)

cps:
	cp main.ps /u/h/a/haryadi/public/html/main.ps

cpf:
	cp main.pdf /u/h/a/haryadi/public/html/main.pdf

clean:
	rm -vf *.ps  main.pdf *.dvi *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png

cleanabit:
	rm -vf *.ps  *.aux \
	*.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png



